Fairness Risks for Group-conditionally Missing Demographics

Fairness-aware classification models have gained increasing attention in recent years as concerns grow on discrimination against some demographic groups. Most existing models require full knowledge of the sensitive features, which can be impractical due to privacy, legal issues, and an individual's fear of discrimination. The key challenge we will address is the group dependency of the unavailability, e.g., people of some age range may be more reluctant to reveal their age. Our solution augments general fairness risks with probabilistic imputations of the sensitive features, while jointly learning the group-conditionally missing probabilities in a variational auto-encoder. Our model is demonstrated effective on both image and tabular datasets, achieving an improved balance between accuracy and fairness.

==> Definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}
%\RequirePackage{eucal}

%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\atil}{{\tilde{a}}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{{\tilde{y}}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\widehat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\widehat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\oobar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sbb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\bA}{\mathbb{A}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bD}{\mathbb{D}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bG}{\mathbb{G}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bJ}{\mathbb{J}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bM}{\mathbb{M}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bO}{\mathbb{O}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bS}{{\mathbb{S}}}
\newcommand{\bT}{{\mathbb{T}}}
\newcommand{\bU}{\mathbb{U}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\bW}{\mathbb{W}}
\newcommand{\bX}{\mathbb{X}}
\newcommand{\bY}{\mathbb{Y}}
\newcommand{\bZ}{\mathbb{Z}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\widehat{\vec{y}}}
\newcommand{\avechat}{\widehat{\vec{a}}}

%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
  \newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
  \def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
  \newenvironment{proof}{\par\noindent{\em Proof:\ }}{\hfill\BlackBox\\[.0mm]}
\fi
%\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}

\ifx\theorem\undefined
  \newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
  \newtheorem{example}{Example}
\fi

\ifx\property\undefined
  \newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
  \newtheorem{lemma}{Lemma}
\fi

\ifx\proposition\undefined
  \newtheorem{proposition}{Proposition}
\fi

\ifx\remark\undefined
  \newtheorem{remark}{Remark}
\fi

\ifx\corollary\undefined
  \newtheorem{corollary}{Corollary}
\fi

\ifx\definition\undefined
  \newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
  \newtheorem{conjecture}{Conjecture}
\fi

\ifx\axiom\undefined
  \newtheorem{axiom}[theorem]{Axiom}
\fi

\ifx\claim\undefined
  \newtheorem{claim}[theorem]{Claim}
\fi

\ifx\assumption\undefined
  \newtheorem{assumption}{Assumption}
  %\newtheorem{assumption}{Postulate}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathrm{arg}\mathop{\mathrm{min}}}
\newcommand*{\argmax}{\mathrm{arg}\mathop{\mathrm{max}}}
\newcommand*{\arginf}{\mathrm{arg}\mathop{\mathrm{inf}}}
\newcommand*{\argsup}{\mathrm{arg}\mathop{\mathrm{sup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}

%\newcommand{\ln}{\mathop{\mathrm{ln}}}
%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
  \newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
  \newcommand{\aleq}{\preccurlyeq}
  \newcommand{\ageq}{\succcurlyeq}
  %%%%%%%% Short Forms %%%%%%%%%%%%%%%

  \newcommand{\ea}{\emph{et al.}}
  \newcommand{\eg}{\emph{e.g.}}
  \newcommand{\ie}{\emph{i.e.}}
  \newcommand{\iid}{\emph{i.i.d.}}
  \newcommand{\cf}{\emph{cf.}\ }
  \newcommand{\wrt}{\emph{w.r.t.}\ }

  %%%%%%%% Brackets %%%%%%%%%%%%%%%

  \newcommand{\rbr}[1]{\left(#1\right)}
  \newcommand{\sbr}[1]{\left[#1\right]}
  \newcommand{\cbr}[1]{\left\{#1\right\}}
  \newcommand{\nbr}[1]{\left\|#1\right\|}
  \newcommand{\abr}[1]{\left|#1\right|}
  \newcommand{\abs}[1]{\left|#1\right|}
  \newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
  \newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
  \newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
  \newcommand{\norm}[1]{\|#1\|}
  \newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
  \newcommand{\sembrack}[1]{[\![#1]\!]}

  %%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

  \newcommand{\one}{\mathbf{1}}  % Identity
  \newcommand{\zero}{\mathbf{0}} % Zero
  \newcommand{\ind}{\boldsymbol{\mathsf{I}}}
  \newcommand{\half}{\frac{1}{2}}
  \newcommand{\sqrttwo}{\sqrt{2}}
  \newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
  \newcommand{\rmd}{\ensuremath{\mathrm{d}}}

  %%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

  \newcommand{\sigmab}{\bm{\sigma}}
  \newcommand{\Sigmab}{\mathbf{\Sigma}}

%   \newcommand{\val}{\vec{\alpha}}
  \newcommand{\vbeta}{\vec{\beta}}
  \newcommand{\vde}{\vec{\delta}}
  \newcommand{\vga}{\vec{\gamma}}
  \newcommand{\vsig}{\vec{\sigma}}
  \newcommand{\vth}{\vec{\theta}}
  \newcommand{\veta}{\vec{\eta}}
  \newcommand{\vnu}{\vec{\nu}}
  \newcommand{\vpsi}{\vec{\psi}}
  \newcommand{\vpi}{\vec{\pi}}
  \newcommand{\vphi}{\vec{\phi}}
  \newcommand{\vxi}{\vec{\xi}}
  \newcommand{\vze}{\vec{\zeta}}
  \newcommand{\vlambda}{\vec{\lambda}}
  \newcommand{\vtheta}{\vec{\theta}}

  \newcommand{\valbar}{\bar{\val}}
  \newcommand{\valhat}{\hat{\val}}
  \newcommand{\valtil}{\tilde{\val}}
  \newcommand{\vthtil}{\tilde{\vth}}
  \newcommand{\vthhat}{\hat{\vth}}
  \newcommand{\vthbar}{\bar{\vth}}
  \newcommand{\vbetatil}{\tilde{\vbeta}}
  \newcommand{\vbetahat}{\hat{\vbeta}}

  \newcommand{\alphavec}{\val}
  \newcommand{\alphavecbar}{\bar{\val}}
  \newcommand{\alphavechat}{\hat{\val}}
  \newcommand{\alphavectil}{\tilde{\val}}
  \newcommand{\betavec}{\vec{\beta}}
  \newcommand{\gammavec}{\vec{\gamma}}
  \newcommand{\deltavec}{\vec{\delta}}
  \newcommand{\etavec}{\vec{\eta}}
  \newcommand{\phivec}{\vec{\phi}}
  \newcommand{\pivec}{\vec{\pi}}
  \newcommand{\psivec}{\vec{\psi}}
  \newcommand{\thetavec}{\vec{\theta}}
  \newcommand{\muvec}{\vec{\mu}}
  \newcommand{\xivec}{\vec{\xi}}
  \newcommand{\chivec}{\vec{\chi}}
  \newcommand{\lambdavec}{\vec{\lambda}}



  \newcommand{\alphab}{\boldsymbol{\alpha}}
  \newcommand{\betab}{\boldsymbol{\beta}}
  \newcommand{\gammab}{\boldsymbol{\gamma}}
  \newcommand{\thetab}{\boldsymbol{\theta}}
  \newcommand{\mub}{\boldsymbol{\mu}}
  \newcommand{\xib}{\boldsymbol{\xi}}
  \newcommand{\Deltab}{\boldsymbol{\Delta}}
  \newcommand{\Pib}{\boldsymbol{\Pi}}
  \newcommand{\etab}{\boldsymbol{\eta}}
  \newcommand{\taub}{\boldsymbol{\tau}}
  \newcommand{\lambdab}{\boldsymbol{\lambda}}
  \newcommand{\rhob}{\boldsymbol{\rho}}

  \newcommand{\delhat}{\hat{\delta}}
  \newcommand{\phihat}{\hat{\phi}}
  \newcommand{\delbar}{\bar{\delta}}
  \newcommand{\alphahat}{\hat{\alpha}}
  \newcommand{\thetahat}{\hat{\theta}}

  \newcommand{\thetabar}{\bar{\theta}}
  \newcommand{\betahat}{\hat{\beta}}
  \newcommand{\Scalhat}{\hat{\Scal}}
  \newcommand{\Scalbar}{\bar{\Scal}}


  \newcommand{\xibar}{\bar{\xi}}
  \newcommand{\mubar}{\bar{\mu}}

  \newcommand{\alphatil}{\tilde{\alpha}}
  \newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
  \newcommand{\thetatil}{\tilde{\theta}}
  \newcommand{\betatil}{\tilde{\beta}}
  \newcommand{\etatil}{\tilde{\eta}}
  \newcommand{\pitil}{\tilde{\pi}}
  \newcommand{\elltil}{\tilde{\ell}}

  %%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

  \newcommand{\BMRM}{{\sf BMRM}}
  \newcommand{\bmrm}{{\sf BMRM}}
  \newcommand{\cpm}{{\sf CPM}}
  \newcommand{\liblinear}{{\sf liblinear}}
  \newcommand{\lsbmrm}{{\sf ls-bmrm}}
  \newcommand{\qpbmrm}{{\sf qp-bmrm}}
  \newcommand{\pegasos}{{\sf pegasos}}
  \newcommand{\pegan}{{\sf pegasos-$n$}}
  \newcommand{\pegaone}{{\sf pegasos-1}}
  \newcommand{\svmstruct}{{\sf SVM-Struct}}
  \newcommand{\svmperf}{{\sf SVM-Perf}}
  \newcommand{\nest}{{\sf pragam}}
  \newcommand{\nestb}{{\sf pragam-b}}
  \newcommand{\mcn}{{\sf M$^3$N}}
  \newcommand{\expgrad}{{\sf ExpGrad}}
  \newcommand{\smo}{{\sf SMO}}
  \newcommand{\lasvm}{{\sf LaSVM}}
  \newcommand{\sms}{{\sf SMS}}


  \newcommand{\prbep}{{\sf PRBEP}}
  \newcommand{\rocarea}{{\sf ROCArea}}

  \newcommand{\arow}[2]{#1_{#2\cdot}}
  \newcommand{\acol}[2]{#1_{\cdot#2}}
  \newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
  \newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
  \newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
  \newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

  \newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
  \def\ci{\perp\!\!\!\perp}

  \newcommand{\ve}{\varepsilon}

  \newcommand{\gstar}{g^{\star}}
  \newcommand{\fstar}{f^{\star}}
  \newcommand{\hstar}{h^{\star}}
  \newcommand{\Astar}{A^{\star}}
  \newcommand{\Kstar}{K^{\star}}

%   \newcommand{\var}{\mathrm{Var}}
  \newcommand{\grad}{{\nabla}}
  \newcommand{\gradtil}{{\tilde{\grad}}}
  \newcommand{\MED}{{\text{MED}}}
  \newcommand{\where}{{\quad \text{where} \quad}}
  \newcommand{\lcg}{{\textit{l.c.g}}}
  \newcommand{\cp}{\mathrm{cp}}
  \newcommand{\err}{{\sf err}}
  \newcommand{\wvechat}{\hat{\vec{w}}}

  \newcommand{\ydiff}[2]{\delta(#1, #2)}
  \newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
  \newcommand{\myfdiff}[2]{\Delta f(#1, #2)}


  \newcommand{\Aone}{\textbf{A1}}
  \newcommand{\Atwo}{\textbf{A2}}
  \newcommand{\supp}{\mathrm{supp}}
  \newcommand{\blue}[1]{\textcolor[rgb]{0.00,0.00,1.00}{#1}}
  \newcommand{\red}[1]{\textcolor[rgb]{1.00,0.00,0.00}{#1}}
  \newcommand{\green}[1]{\textcolor[rgb]{0.00,1.00,0.00}{#1}}
  \newcommand{\black}[1]{\textcolor[rgb]{0.00,0.00,0.00}{#1}}
  \newcommand{\vardef}{\stackrel{\triangle}{=}}
  \newcommand{\smallonevec}{{\scriptsize\mathbf 1}}
  \newcommand{\smallwvec}{{\scriptsize\mathbf w}}
  \newcommand{\smallqvec}{{\scriptsize\mathbf q}}
  \newcommand{\smallyvec}{{\scriptsize\mathbf y}}
  \newcommand{\smallepsvec}{{\mbox{\boldmath\scriptsize $\epsilon$}}}
  \newcommand{\smallzetavec}{{\mbox{\boldmath\scriptsize $\zeta$}}}
  \newcommand{\smallmuvec}{{\mbox{\boldmath\scriptsize $\mu$}}}
  \newcommand{\smallnuvec}{{\mbox{\boldmath\scriptsize $\nu$}}}
  \newcommand{\smallxivec}{{\mbox{\boldmath\scriptsize $\xi$}}}
  \newcommand{\smalllambdavec}{{\mbox{\boldmath\scriptsize $\lambda$}}}
  \newcommand{\smallthetavec}{{\mbox{\boldmath\scriptsize $\theta$}}}
  \newcommand{\smallalphavec}{{\mbox{\boldmath\scriptsize $\alpha$}}}
  \newcommand{\smallbetavec}{{\mbox{\boldmath\scriptsize $\beta$}}}
  \newcommand{\smalletavec}{{\mbox{\boldmath\scriptsize $\eta$}}}
  \newcommand{\smallomegavec}{{\mbox{\boldmath\scriptsize $\omega$}}}
  \newcommand{\smallLambdavec}{{\mbox{\boldmath\scriptsize $\Lambda$}}}
  \newcommand{\epsvec}{{\mbox{\boldmath $\epsilon$}}}
  \newcommand{\ellvec}{{\mbox{\boldmath $\ell$}}}
  \newcommand{\nuvec}{{\mbox{\boldmath $\nu$}}}
  \newcommand{\sigmavec}{{\mbox{\boldmath $\sigma$}}}
  \newcommand{\omegavec}{{\mbox{\boldmath $\omega$}}}
  \newcommand{\zetavec}{{\mbox{\boldmath $\zeta$}}}
  \newcommand{\sign}{{\textrm{sign}}}
  \newcommand{\hinge}{{\textit{hinge}}}
  \newcommand{\loss}{{\textit{loss}}}
  \newcommand{\etahinge}[1]{{{#1}\mbox{-}\hinge}}
  \newcommand{\robust}{{\textit{robust}}}
  %\newcommand{\regrobust}{{f_{\scriptsize\textit{robust}}}}
  \newcommand{\regrobust}{{f_{\scriptsize\textit{rob}}}}
  %\newcommand{\regetahinge}{{f_{\scriptsize\textit{hinge}}}}
  \newcommand{\regetahinge}{{f_{\scriptsize\textit{hng}}}}
  \newcommand{\looerr}{{\textit{loo\_err}}}
  \newcommand{\makevector}[1]{{\mathbf #1}}
  \newcommand{\Ker}{\ensuremath{\mathrm{Ker}}}
  \newcommand{\Img}{\ensuremath{\mathrm{Im}}}




  \newcommand{\smax}{\mathop{\mathrm{smax}}}
  \newcommand{\indmax}{\mathop{\mathrm{indmax}}}
  \newcommand{\McalML}{\mathop{\Mcal_{\mathrm{ML}}}}
  \newcommand{\McalMLeps}{\mathop{\Mcal^{\epsilon}_{\mathrm{ML}}}}
  \newcommand{\McalMLn}{\mathop{\Mcal^{1}_{\mathrm{ML}}}}

  %\newcommand{\cvxind}{$\text{CVX}_{\text{ind}}$}
  %\newcommand{\cvxtrans}{$\text{CVX}_{\text{trans}}$} 

  \newcommand{\fstartil}{\tilde{f^*}}
  \newcommand{\gstartil}{\tilde{g^*}}
  \newcommand{\Bcaltil}{{\tilde{\Bcal}}}
  \newcommand{\sip}{{s.i.p.}}
  \newcommand{\sipsf}{{{\sf Embed}}}
  \newcommand{\vanilla}{{{\sf Vanilla}}}
  \newcommand{\mlsvm}{{{\sf ML-SVM}}}
  \newcommand{\hrsvm}{{{\sf HR-SVM}}}
  \newcommand{\gws}{{GW_\Scal}}
  \newcommand{\gw}{\textsf{GW}}
  \newcommand{\fgw}{\textsf{FGW}}
  \newcommand{\ogw}{\textsf{OGW}}
  \newcommand{\ofgw}{\textsf{OFGW}}
  % \newcommand{\gwtil}{\widetilde{GW}}
  % \newcommand{\fgwtil}{\widetilde{FGW}}
  \newcommand{\fgwtila}{\widetilde{FGW}_{\!\Acal}}
  \newcommand{\fgwu}{{FGW}_{\!u}}
  \newcommand{\gwu}{{GW}_{\!u}}
  \newcommand{\Omegabar}{\bar{\Omega}}
  \newcommand{\Lambdahat}{\hat{\Lambda}}
